A Fine-Grained Classification of the Complexity of Evaluating the Tutte Polynomial on Integer Points Parameterized by Treewidth and Cutwidth

We give a fine-grained classification of evaluating the Tutte polynomial $T(G;x,y)$ on all integer points on graphs with small treewidth and cutwidth. Specifically, we show for any point $(x,y) \in \mathbb{Z}^2$ that either - can be computed in polynomial time, - can be computed in $2^{O(tw)}n^{O(1)}$ time, but not in $2^{o(ctw)}n^{O(1)}$ time assuming the Exponential Time Hypothesis (ETH), - can be computed in $2^{O(tw \log tw)}n^{O(1)}$ time, but not in $2^{o(ctw \log ctw)}n^{O(1)}$ time assuming the ETH, where we assume tree decompositions of treewidth $tw$ and cutwidth decompositions of cutwidth $ctw$ are given as input along with the input graph on $n$ vertices and point $(x,y)$. To obtain these results, we refine the existing reductions that were instrumental for the seminal dichotomy by Jaeger, Welsh and Vertigan~[Math. Proc. Cambridge Philos. Soc'90]. One of our technical contributions is a new rank bound of a matrix that indicates whether the union of two forests is a forest itself, which we use to show that the number of forests of a graph can be counted in $2^{O(tw)}n^{O(1)}$ time.

==> HaLowerbound.tex <==
We trivially get the following lower bound from existing bounds on the non-parameterized version of the problem \cite{Dell_2014}.
\begin{theorem} \label{thm:HaLow}
    Computing the Tutte polynomial along the curve $H_\alpha$ cannot be done in time $O(2^{o(\ctw)} n^{O(1)})$, unless \textsc{\#ETH} fails.
\end{theorem}
\textcolor{red}{????} \\
\textcolor{blue}{Interpolation with flow polynomial?} \\
\textcolor{blue}{Use structure of constant cutwidth graph to show you need fewer points.} \\
\textcolor{blue}{Compute chromatic polynomials of bags and then somehow reconstruct for the whole graph. Related to polynomial reconstruction from the polynomial deck.} \\
\textcolor{blue}{Block Interpolation.}
\textcolor{blue}{Use reduction from \url{https://arxiv.org/pdf/1206.1775.pdf}, but to $\tw$-pair multicut.}

\subparagraph{Reduction to minimal $\tw$-terminal multicut}
\textcolor{red}{Potential issue: we need to ensure that every minimal multicut has the same number of components. For multiway cut this follows from minimality, but for multicut this is not (necessarily) the case.}
